QiMeng-PRepair: Precise Code Repair via Edit-Aware Reward Optimization

Large Language Models (LLMs) achieve strong program repair performance but often suffer from over-editing, where excessive modifications overwrite correct code and hinder bug localization. We systematically quantify its impact and introduce precise repair task, which maximizes reuse of correct code while fixing only buggy parts. Building on this insight, we propose PRepair, a framework that mitigates over-editing and improves repair accuracy. PRepair has two components: Self-Breaking, which generates diverse buggy programs via controlled bug injection and min-max sampling, and Self-Repairing, which trains models with Edit-Aware Group Relative Policy Optimization (EA-GRPO) using an edit-aware reward to encourage minimal yet correct edits. Experiments show that PRepair improves repair precision by up to 31.4% under $\mathrm{fix}_1@1$, a metric that jointly considers repair correctness and extent, and significantly increases decoding throughput when combined with speculative editing, demonstrating its potential for precise and practical code repair.

==> section/1-introduction-1226.tex <==
\section{Introduction}
\label{sec:intro}

\iffalse

\fi



% 一、代码修复背景
% 1. 定位、检索、修复、验证的多阶段
% 2. 编程助手催生了端到端训练模型修复代码的工作
Program repair aims to automatically correct faulty programs while preserving their intended semantics, and has become an important research area in the era of Large Language Models~\citep{qwen25coder,surveyofapr,surveybenchmarkssolutions}. 
Prior works generally follows a structured paradigm, decomposing the task into stages such as error localization, correction, and validation~\citep{agentless,verilogcoder,Epperson_2025}. 
With the growing use of coding assistants like Copilot and Cursor, there is an increasing need for fast, end-to-end program repair models. 
To address this demand, many recent approaches employ supervised fine-tuning (SFT) and reinforcement learning (RL) to train models capable of performing program repair accurately.

\begin{figure}[t]
  \includegraphics[width=\linewidth]{figures/first.pdf}
  \caption {Compare Prepair’s repair performance with other models. Existing models suffer from \textbf{Over-editing}, which not only reduces repair accuracy but also significantly increases the review burden for developers.}
   \label{fig:1} 
\end{figure}
% 二、存在over-editing问题（现有工作的缺陷）
% 1. 只考虑正确性丧失了精准修复能力，进而无法进一步提升修复能力
% 2. over-editing影响了维护性，速度

%Rui
%第2段
%现有工作只考虑正确性，并不能精确的修复错误
%我们命名为over-editing现象
%结合fig1描述over-editing现象是什么
%over-editing的坏处，①无法定位错误，②破坏原有的代码逻辑，不易维护，实际使用中不够友好
%precise repair更加合理，（精确修复的定义）最大化复用现有代码，（优势）这既有助于保持代码质量，也能减轻开发者的审阅负担
%总结，研究precise repair是important but remains an unsolved issue
%第3段
%precise repair的challenge
%①数据稀缺：没有带错误定位的数据
%②正确代码保持：如何在修复时不修改正确的部分，仅对错误进行修复

Training LLMs for code repair faces two key challenges: (1) Data challenge. Effective repair requires models to understand the semantics of buggy programs, reuse their correct components, and precisely localize and fix errors. However, realistic buggy code that simultaneously contains substantial correct logic and localized faults is extremely scarce. (2) Algorithmic challenge. Most existing approaches~\citep{humanevalfix,qwen25coder,morepair,slmfix} optimize repair correctness alone, treating code repair as a correctness-only objective. This formulation ignores how much the model modifies the original program, which is a crucial dimension for repair that reflects program understanding and directly affects readability and maintainability. As a result, we observe a pronounced \textit{over-editing} phenomenon, where models increasingly diverge from the original semantics during training and may even rewrite the entire program (Figure~\ref{fig:1}). Over-editing effectively collapses code repair into code generation, undermining error localization and producing unnecessarily large patches that are difficult to review. This issue is particularly problematic for practical coding assistants such as Cursor: when speculative edits are integrated, over-editing reduces the acceptance rate and consequently degrades throughput~\citep{cursor}.

% Existing training approaches focus primarily on repair correctness~\citep{humanevalfix,qwen25coder,morepair,slmfix} while largely ignoring the number of edits required to achieve a correct fix. We observe that this can lead to an \textit{over-editing} phenomenon, where the model increasingly diverges from the original program’s semantics during training and may even rewrite the entire program (see Figure \ref{fig:observation}). This phenomenon introduces two major issues: (1) Undermines the implicit ability for error localization. If a model rewrites the entire program without preserving the original logic, it no longer performs genuine repair but behaves like code generation. Such training encourages superficial rewriting and weakens the model’s ability to understand programs and precisely locate errors. (2) Affects code maintainability. An effective repair should reuse as much existing code as possible, which preserves code quality and reduces the review burden for developers. This is particularly important in real-world settings where coding assistants, such as Cursor, are widely used (as shown in Figure~\ref{fig:1}). Moreover, for systems like Cursor that integrate speculative editing, more precise repairs can also lead to faster repair speed~\citep{cursor}.

% 三、我们的insight，提出的方法，解决的问题

To address these challenges, we propose the \textbf{PRepair} framework, which alleviates data scarcity in code repair and explicitly guides models to perform precise repairs. Our central insight is that optimizing for minimal yet sufficient edits preserves repair correctness while encouraging faithful reuse of correct program logic. The PRepair framework consists of two steps: (1) \textit{Self-Breaking}, where we design a precise code repair data generation framework that introduces bugs into correct programs to create large-scale training data, combined with a min–max sampling strategy to reduce data volume while preserving the diversity of buggy programs; (2) \textit{Self-Repairing}, where the model is optimized using EA-GRPO to encourage both correct and minimal code repairs. EA-GRPO incorporates an edit-aware reward, where edit penalties are applied only after the model achieves sufficient repair correctness. This design effectively balances repair correctness and precision, encouraging minimal yet accurate code fixes. To evaluate both repair correctness and the extent of modifications, we introduce $\mathrm{fix}_p@k$, the first metric specifically designed for assessing code repair, which jointly considers correctness and the number of edits.

% To address these issues, we propose the \textbf{PRepair} framework, which is designed to improve program repair capability while mitigating the over-editing problem. The PRepair framework consists of two steps: (1) \textit{Self-Breaking}, where the model introduces bugs into correct programs to generate large scale training data. We further apply a min–max sampling strategy to reduce data volume while preserving the diversity of buggy programs; (2) \textit{Self-Repairing}, where the model is optimized using Group Relative Policy Optimization (GRPO) with Dynamic Editing Penalty (DEP) to encourage correct and minimal code repairs. DEP introduces an accuracy-aware reward mechanism, where edit penalties are applied only after the model achieves sufficient repair correctness. This design balances repair accuracy and repair precision, encouraging minimal yet correct code fixes. 


% 三、算法优势
Compared with previous methods that optimize code repair solely for correctness, our method offers two key advantages. First, the model learns to focus its attention on the buggy lines, acquiring an implicit error localization ability that guides precise repair. Second, by following the logic of the buggy code, it reuses correct portions of the original program, which not only improves repair accuracy but also enhances cross-domain code repair capability.

% 四、实验效果，正确性，fix_p，修复速度
Experiments across multiple models and benchmarks show that PRepair effectively reduces unnecessary code edits while improving repair correctness. Moreover, PRepair can be combined with speculative editing techniques to enable faster inference, which provides practical benefits for developers in real-world programming scenarios. The main contributions of this paper are as follows:

% 五、贡献

% 1. benchmark, Full-Stack Fixbench，第一个跨编程范式代码修复
% 2. 评估指标，fix_p 综合衡量编辑代价与正确性的指标
% 3. 实验效果，DEP 算法，相比 naive GRPO 在 Full-Stack Fixbench 效果均更好

\begin{itemize}
\item We systematically analyze the over-editing behavior of LLMs and find that it becomes more pronounced when trained with GRPO using the Correctness Reward.
\item We propose the \textbf{PRepair} framework, which enhances code repair without requiring labeled data. EA-GRPO, an RL-based method, is leveraged to train models that make precise and minimal edits.
% \item We introduce the $\mathrm{fix}_p@k$ metric, the first evaluation metric specifically designed for code repair, which jointly measures repair correctness and precision.
\item Empirical evaluations on multiple benchmarks demonstrate the effectiveness and superior performance of our proposed EA-GRPO.
\item When integrating speculative edits, model trained with EA-GRPO achieves a 15\% increase in throughput, highlighting the practical value for real-world code assistance deployment.
\end{itemize}
